Assessing Code Authorship: The Case of the Linux Kernel

Code authorship is a key information in large-scale open source systems. Among others, it allows maintainers to assess division of work and identify key collaborators. Interestingly, open-source communities lack guidelines on how to manage authorship. This could be mitigated by setting to build an empirical body of knowledge on how authorship-related measures evolve in successful open-source communities. Towards that direction, we perform a case study on the Linux kernel. Our results show that: (a) only a small portion of developers (26 %) makes significant contributions to the code base; (b) the distribution of the number of files per author is highly skewed --- a small group of top authors (3 %) is responsible for hundreds of files, while most authors (75 %) are responsible for at most 11 files; (c) most authors (62 %) have a specialist profile; (d) authors with a high number of co-authorship connections tend to collaborate with others with less connections.

==> discussion.tex <==
\section{Summary of Results}
\label{sec:discussion}

We set to extract various parameters of how authorship works in the Linux 
kernel evolution. As such, we ask four research questions.

When answering RQ.1 (proportion of authors), we find that $27\,\%$ of developers 
are authors---the heavy-workload in the Linux kernel evolution is in the hands 
of less than a third of all its developers. At the subsystem level, not all 
subsystems follow the same parameter. It appear to do so whenever 
the subsystem depends on vendor-specific code (e.g, as in \emph{Arch} 
and \emph{Driver}) or relates to the "brain" of the kernel (e.g., 
as in \emph{Core}).

Our investigation of RQ.2 (number of files/author) finds that the number of 
files per author is highly 
skewed across all releases, but it is becoming more equal with time. We also 
find that Linus is becoming more benevolent, decentralizing authorship to 
other top-authors. This is indeed require for the kernel to continue evolving 
at a fast pace. Up to the $75\,\%$ percentile, the global distribution and the 
ones we find in \emph{Fs}, \emph{Arch}, \emph{Driver}, and \emph{Net} 
are very similar. Still, the global parameter does not fully represent the 
number of files per author in \emph{Core} and \emph{Misc}.

The results we find for RQ.3 (work specialization) shows that the Linux kernel 
architectural 
decomposition partially fosters work specialization. It definitely does so for 
the \emph{Driver} subsystem (relatively independent from other parts of the 
kernel), but less so in other subsystems.

Last, but not least, RQ.4 (co-authorship properties) we find that on average, 
maintaining a file in Linux is 
requires at least 3 authors. Such average seems constant over time. 
Moreover, the co-authorship network indicates that authors that collaborate 
with many other do so in a way to "help" authors who collaborate less, 
suggesting some sort of mentor ship.

